Can Knowledge of End-to-End Text-to-Speech Models Improve Neural MIDI-to-Audio Synthesis Systems?

With the similarity between music and speech synthesis from symbolic input and the rapid development of text-to-speech (TTS) techniques, it is worthwhile to explore ways to improve the MIDI-to-audio performance by borrowing from TTS techniques. In this study, we analyze the shortcomings of a TTS-based MIDI-to-audio system and improve it in terms of feature computation, model selection, and training strategy, aiming to synthesize highly natural-sounding audio. Moreover, we conducted an extensive model evaluation through listening tests, pitch measurement, and spectrogram analysis. This work demonstrates not only synthesis of highly natural music but offers a thorough analytical approach and useful outcomes for the community. Our code, pre-trained models, supplementary materials, and audio samples are open sourced at https://github.com/nii-yamagishilab/midi-to-audio.

==> data.tex <==
\section{NII-URMP Dataset (temporary)}\label{sec:database}

High-quality data is one of the most essential factors for data-driven algorithms.  To synthesis natural multi-instrument audio, we take URMP Database \cite{li2018creating} as prototype and record a new database named \newdata for better MIDI and audio alignment, higher quality of audio, and more practical testing scenario on unseen instruments.  

In \newdata, we follow repertoires and recording settings in \cite{li2018creating} to separately record individual tracks from 44 pieces of performance.  To facilitate the music synthesis and music transcription, MIDI and audio are aligned in high accuracy by xxx so that the lapse between music score and audio is generally less than xx ms. \textcolor{cyan}{Xuan: how to record the dataset to control the alignment accuracy?}  We invite professional musicians to perform high quality music pieces in both expression and accuracy.  Shown in the Table \ref{tab: nii-urmp corpos statistic}, not all instrument categories in valid and test sets exist in the training set: Contrabass in valid set is unnseen to the training set, while Flugelhorn, Soprano Saxophone in test set are unseen.  The unseen instrument categories provide good opportunities to evaluate the generalization ability of synthesis model. 


\begin{table*}[!t]
\caption{Statistics of training, validation, and test sets extracted from NII-URMP corpus.  \textit{Dur} denotes duration in minutes.  $\text{MIDI}_\text{max}$ and $\text{MIDI}_\text{min}$ denote maximum and minimum MIDI notes, respectively. The validation set's unseen instrument is the Flugelhorn and Soprano Saxophone, and the test set's unseen instrument is the Contrabass.  The validation set contains about 54 minutes of data.  The test set contains about 49 minutes of data.}
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2pt}
\scalebox{0.93}{
\begin{tabular}{l|cccc|cccc|cccc}
\hline\hline
      & \multicolumn{4}{c|}{Training set} & \multicolumn{4}{c|}{Validation set} & \multicolumn{4}{c}{Test set} \\
      & \multicolumn{4}{c|}{97 music pieces} & \multicolumn{4}{c|}{22 music pieces} & \multicolumn{4}{c}{30 music pieces} \\
\cline{2-13}
     & \# & \textit{Dur}. & $\text{MIDI}_\text{max}$ & $\text{MIDI}_\text{min}$ 
     & \# & \textit{Dur}. & $\text{MIDI}_\text{max}$ & $\text{MIDI}_\text{min}$
     & \# & \textit{Dur}. & $\text{MIDI}_\text{max}$ & $\text{MIDI}_\text{min}$ \\
\hline
Violin & 23 & 41.36 & 90 & 56 & 9 & 20.16 & 83 & 56 & 2 & 4.62 & 83 & 56  \\
Violincello & 8 & 18.25 & 68 & 37 & 2 & 4.48 & 60 & 37 & 1 & 2.32 & 63 & 39  \\
Viola & 7 & 16.63 & 78 & 49 & 5 & 11.18 & 73 & 51 & 1 & 2.32 & 70 & 50 \\
Contrabass & – & – & – & – & 3 & 6.79 & 58 & 34 & – & – & – & –  \\
Flute & 8 & 13.01 & 94 & 61 & 1 & 2.18 & 83 & 63 & 9 & 14.79 & 95 & 66  \\
Oboe & 1 & 2.14 & 87 & 68 & - & - & - & - & 5 & 8.55 & 83 & 59   \\
Clarinet & 6 & 9.60 & 82 & 51 & 1 & 2.19 & 70 & 51 & 3 & 5.46 & 82 & 55  \\
Flugelhorn & - & - & - & - & - & - & - & - & 3 & 3.88 & 68 & 44  \\
Horn & 4 & 7.56 & 72 & 48 & - & - & - & - & 1 & 2.34 & 70 & 50  \\
Trumpet & 19 & 36.31 & 82 & 53 & - & - & - & - & 2 & 4.67 & 83 & 54  \\
Trombone & 8 & 14.71 & 68 & 41 & - & - & - & - & 1 & 2.34 & 66 & 41  \\
Tuba & 5 & 8.72 & 56 & 30 & - & - & - & - & - & - & - & - \\
Soprano Saxophone & - & - & - & - & - & - & - & - & 2 & 3.09 & 82 & 58 \\
Alto Saxophone & 5 & 6.50 & 80 & 52 & 1 & 2.30 & 72 & 56 & - & - & - & -  \\
Tenor Saxophone & 3 & 3.46 & 69 & 45 & - & - & - & - & - & - & - & - \\
\hline\hline
\end{tabular}
}
\end{center}
\label{tab: nii-urmp corpos statistic}
\end{table*}

==> deprecated/introduction.tex <==
\section{Introduction}\label{sec:introduction}


Synthesizing music audio from music notes is an essential step in professional music industry, which also plays an important role in music education for beginners.  Traditional sample-based and physical-model-based synthesizers are commonly used in music creation. With the development of deep learning, more and more neural network based algorithms \cite{kim2019neural, cooper2021midi, wu2022mididdsp, dong2022deepperformer} are proposed to synthesize music with better quality, assisting users in fantastic music creation.  

\textcolor{cyan}{NOTE: (Xuan) Sorry I think the current story is too weak. I will rewrite it. Welcome to any suggestion and idea!}
From the audio synthesis perspective, both midi-to-audio and text-to-speech (TTS) are the transform from discrete symbolic data to continuous acoustic data. Therefore, several literature borrow ideas from TTS and apply them to midi-to-audio synthesis.  Cooper \textit{et al.} \cite{cooper2021midi} set up the initial work by adapting the Tacotron \cite{wanv2017tacotron, yasuda2019investigation} and Neural Source-Filter waveform model (NSF) \cite{wang2019neural} to synthesis music with the time-aligned MIDI input.  Similar with \cite{cooper2021midi}, Deep Performer \cite{dong2022deepperformer} modified the FastSpeech \cite{ren2019fastspeech}, a popular TTS acoustic model, to generate spectrum from music score input, and then adopted a well-trained HiFi-GAN \cite{kong2020hifi} to synthesis audio.  Wu \textit{et al.} proposed MIDI-DDSP which contains three separate modules: Expression Generator, Synthesis Generator, and DDSP Inference \cite{Engel2020DDSP}, to synthesis controllable, expressive, and high fidelity music from music score input.

Recently, an increasing number of synthesis algorithms \cite{kim2021conditional} prove that joint training of the acoustic model and vocoder are prone to have better performance in listening test than the separately trained models, because the mismatch between generated acoustic feature and natural acoustic feature can be eliminated in the end-to-end synthesis paradigm.  Therefore, it is worthwhile to think about: will the cross-model joint training also improve the performance of midi-to-audio synthesis? Another key point in midi-to-audio is about the music score input. Since there are a variety of musical score formats, we are curious about how to adapt the system to different formats of musical score input at a minimum cost.

To address the two problems in the preceding paragraph, we made two improvements on the current midi-to-audio system: 
1) developing the joint training of acoustic model and synthesizer to seek for better quality of synthesized audio; 
2) transforming different types of MIDI signal into a unified intermediate representation as the input of acoustic model.
Our improved system are able to generate more natural audio pieces with different formats of midi signal input.

Contributions (New):
1) joint-training to improve synthesised audio quality (Q: mismatch between generated spectrogram and natural, blurry)
2) multi-instrument audio dataset (Q: we need high quality multi-instrument playing dataset)
3) timbre match loss for higher timbre similarity (low similarity between generated m-i audio and natural, need more regularization)

The structure of the paper is the following: we elaborate on the midi-to-audio system design in Section \ref{sec:methods} and introduce the details of model implementation, evaluation metrics, and models’ performance in Section \ref{sec:experiments}.



==> deprecated/methods.tex <==
\section{Methods}\label{sec:methods}

The multi-instrument audio synthesis system takes midi signal and instrument embeddings as input and synthesis music audio.   Architecture of the system is shown in Fig. \ref{}.  The model is trained jointly to improve audio's naturalness and regularized with timbre match loss to increase the similarity of timbre between synthesized audio and natural audio.

\subsection{MIDI-to-Audio}

Text-to-Speech (TTS) and MIDI-to-Audio both take compact symbolic sequences as input and synthesis audio waveforms, which allow them to share mechanisms and techniques in many aspects, such as spectrogram modeling, waveform generation, and training strategy.  One of the most popular deep learning based TTS paradigm is generating mel-spectrogram from phoneme input sequence with acoustic model and synthesis audio from mel-spectrogram with waveform model.  The waveform model is trained with natural mel-spectrogram input, while is inferenced with generated spectrogram from acoustic model.  The mismatch between synthesized and natural spectrogram lead to the potential audio quality degradation.  To solve this problem, jointly trained end-to-end TTS models are proposed to eliminate the mismatch between the waveform model input in the different phases, which arouses our interests to improve the quality of music synthesis based on similar training strategy.

Joint-training in speech and music synthesis refers to generating audio from symbolic input end-to-end by updating parameters of acoustic model and waveform model together.  Spectrogram, formal output of acoustic model and input of waveform model, is taken as intermediate  variable of the joint synthesis model.  However, considering the joint model is composed with acoustic model and waveform model, large sub-model significantly lag out the training and inference speed of the joint model and lead to memory issues.  Therefore, it is necessary to adopt computation-saving acoustic model and waveform model in the joint training without too much sacrifice on quality performance.  

Neural network-based acoustic models, such as Tacotron \cite{wanv2017tacotron} and Transformer-TTS \cite{li2019neural}, have gradually replaced traditional statistical-based acoustic models due to their impressive performance of the synthesised audio.  In TTS tasks, both Tacotron and Transformer transform phoneme input to hidden state with encoder and auto-regressively generate spectrogram with hidden state and ground truth input by the decoder.  Similarly, in midi-to-audio tasks, we replace the symbolic input from phoneme sequence to pianoroll sequence.  Considering the complexity of music melody, we adopt a linear layer to transform the input pianoroll into embeddings for encoder.  Moreover, we follow \cite{cooper2021midi} to take the MIDI-Spectrogram as object of acoustic models because the correspondence between MIDI-Spectrogram and pianoroll helps acoustic model to converge faster.  Compared with RNN-based Tacotron, attention-based Transformer-TTS is preferable in joint training because of its comparable audio quality but higher computation efficiency \cite{li2019neural}. 

% \textcolor{cyan}{[Xuan: is it better to name our vocoder? such as synthesizer or spectrogram inverter]} 
Transforming MIDI-Spectrogram to audio waveform is another important stage in the music synthesis.  We utilize well-performed waveform models in TTS, such as, NSF \cite{wang2019neural}, NSF-GAN, and HiFi-GAN \cite{kong2020hifi} to synthesis music audio.  One of the most challenging problems are adapting NSF designed for monophonic speech to polyphonic music synthesis.  Inspired by \cite{cooper2021midi, wang2019neural}, we take noise as excitation signal in the NSF training and employ NSF-GAN with discriminator to synthesis more realistic audio by adversarial training.  


\subsection{Multi-Instrument Audio Synthesis}

Inspired with zero-shot multi-speaker text-to-speech synthesis \cite{cooper2020zero}, we develop the multi-instrument audio synthesis system based on the aforementioned midi-to-audio technology guided by the instrument embeddings to synthesis music audio from different instrument. 

We utilize the instrument encoder from \cite{shi2022instr} to extract musical instrument embeddings.  The instrument encoder in \cite{shi2022instr} adopted SincNet \cite{Ravanelli18SincNet}, ResNet \cite{He16ResNet}, Learnable Dictionary Encoder(LDE) \cite{Cai18LDE}, and other algorithms in order to generate discriminative embeddings for musical instruments.  Taking a piece of raw waveform as input, the CQT-initialized SincNet firstly transforms waveform into spectrogram-like acoustic feature.  Then, ResNet-based backbone extracts frame-level representation from the acoustic feature. And the representation is finally processed to time-invariant 512-D instrument embeddings with LDE.

Shown in the figure, \textcolor{cyan}{NOTE (Xuan): add architecture figure} the instrument embeddings processed with two trainable linear layers are concatenated with the output of acoustic model's encoder, importing the instrument timbre information to the acoustic model decoder.  
In order to improve the timbre similarity of the synthesised audio, we develop the timbre match loss to add regularization on the optimization of acoustic model.  The calculation of timbre match loss is shown following:
\begin{equation}
    \mathcal{L_T} = \mathcal{L}[ E(\hat{y}), E(y)] = \mathcal{L}[ E(\mathbf{G} (x)), E(y)]
\end{equation}
where $\hat{y}$ and $y$ denote synthesised audio waveform from $x$ and the natural waveform, while $E$ and $\mathbf{G}$ denote the instrument encoder and the trainable synthesis system, respectively, including acoustic model and vocoder.  Acoustic model is optimized with $\mathcal{L_T}$ to minimize the cosine distance between the synthesised audio and natural audio.
Apart from guiding acoustic model for synthesis and calculating the timbre matching loss, the instrument embeddings is further employed as a evaluation metrics to measure the timbre similarity between synthesised audio and the natural audio.



